On the Topology Awareness and Generalization Performance of Graph Neural Networks

Many computer vision and machine learning problems are modelled as learning tasks on graphs where graph neural networks GNNs have emerged as a dominant tool for learning representations of graph structured data A key feature of GNNs is their use of graph structures as input enabling them to exploit the graphs inherent topological properties known as the topology awareness of GNNs Despite the empirical successes of GNNs the influence of topology awareness on generalization performance remains unexplored, particularly for node level tasks that diverge from the assumption of data being independent and identically distributed IID The precise definition and characterization of the topology awareness of GNNs especially concerning different topological features are still unclear This paper introduces a comprehensive framework to characterize the topology awareness of GNNs across any topological feature Using this framework we investigate the effects of topology awareness on GNN generalization performance Contrary to the prevailing belief that enhancing the topology awareness of GNNs is always advantageous our analysis reveals a critical insight improving the topology awareness of GNNs may inadvertently lead to unfair generalization across structural groups which might not be desired in some scenarios Additionally we conduct a case study using the intrinsic graph metric the shortest path distance on various benchmark datasets The empirical results of this case study confirm our theoretical insights Moreover we demonstrate the practical applicability of our framework by using it to tackle the cold start problem in graph active learning

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tex_content/paper/fairness.tex <==

\section{A Fair Training Set Sampling Scheme}\label{sec:data_labelling}
We next present an application of our derived results to a sampling scheme for the training/label set that yields a more fair prediction performance of GNNs with respect to graph distance. We have shown that the predictive power of GNNs is closely related to the coverage of the training set. Therefore, the general principle is that we want the training data to have good graph distance coverage on the rest of the data. This can be formulated into the following optimization problem.


\begin{equation}\label{eq:trainSet_selection1}
	\begin{split}
		\min_{\trainSet} \sum_{u \in \mathcal{V} - \trainSet} & d(u, \trainSet)\\
		s.t.  \|\trainSet\| = k
	\end{split}
\end{equation}

\begin{equation}\label{eq:max_cover}
	\begin{split}
		& \max_{\mathcal{D} \subset \mathcal{V}} \sum_{u \in \mathcal{V}\setminus \mathcal{D}} I_r(u|\mathcal{D}) \\
		s.t.& ~~~ |\mathcal{D}| \leq k\\
	\end{split}
\end{equation}
where $k$ is the given initial set size and $r$ is the given neighbourhood radius. $I_r(u|\mathcal{D})$ is an indicator function: $I_r(u|\mathcal{D}) = 1$ if there exists a vertex $v \in \mathcal{D}$ such that $u \in \mathcal{N}_r(v)$, and $I_r(u|\mathcal{D}) =0$, otherwise. The problem can be reduced to the maximal coverage problem~\citep{approx} and the reduction can be found in the supplemental material. The maximal coverage problem is NP-hard. There exist efficient greedy algorithms to achieve an approximation ratio of $1-\frac{1}{e}$, e.g., by selecting a vertex whose neighbour has the most uncovered vertexes at each stage~\citep{approx}. We refer to this selection strategy as the locality-based selection.

We provide an evaluation on the initial set selected by solving (\ref{eq:max_cover}) using the greedy algorithm in \citep{approx}. We compare with the following baselines in the experiment: 1) Uniform Random Sampling (R); 2) Importance Based Sampling (sampling nodes based on node properties such as degree: ID, centrality: IC, and clustering coefficient: ICC). We use the default formulas provided by Networkx~\citep{networkx} to compute these node properties. We apply each strategy to select an initial dataset of 0.5 \% of the size of the largest connected component for labelling (training). We evaluate the classification using the rest of the vertexes. As shown in Table~\ref{tab:init_label}, our strategy consistently outperforms other strategies. 

Our results (Table~\ref{tab:init_label}) suggest that locality-based selection achieves a significant improvement of model performance over the other strategies across different datasets, giving a better kick-start to the active learning process of GNNs.

\begin{table*}[!h]
  \vspace{-3mm}
  \centering
  \caption{ Initial data labelling
  }  
  
  {\small
   \setlength\tabcolsep{1.5pt}
    \begin{tabular}{c|cccc|cccc}
    \toprule
              &        \multicolumn{4}{c}{GCN}              & \multicolumn{4}{c}{Sage}            \\
    \midrule
          &   Cora & CiteSeer & CoraFull & Coauthor CS & Cora & CiteSeer & CoraFull & CoauthorCS\\
    \midrule
    R  & 37.08 (0.41)   &  36.35 (0.74) & 8.13 (0.06) & 57.75 (0.57)    & 37.69 (0.39)& 37.24 (0.42) & 8.56 (0.04) & 49.72 (0.40) \\
    ID  & 40.87 (0.38)  &  36.27 (0.55) & 10.68 (0.04) & 51.50 (0.81)  & 38.04 (0.40) &   35.26 (0.43) &   11.56 (0.03) & 42.78 (1.38)   \\
    IC & 37.81 (1.23)   &  41.02 (0.55) & 10.34 (0.08) & 52.57 (0.62) & 42.11 (1.25)   &  40.74 (0.50) & 10.75 (0.05) & 52.16 (0.58) \\
    ICC  & 40.90 (0.39)   &  37.31 (0.74) & 9.27 (0.10) & 50.98 (0.55) & 38.92 (0.29)  &  40.73 (0.46) & 9.32 (0.05) & 51.85 (0.31)  \\
    OURS  & \textbf{49.03 (0.05)}  &  \textbf{50.98 (0.04)} & \textbf{15.25 (0.00)} & \textbf{61.75 (0.08)}  & \textbf{58.57 (0.01)}  &  \textbf{48.80 (0.00)} & \textbf{14.76 (0.00)} & \textbf{61.63 (0.04)}    \\
    
     \midrule
         & \multicolumn{4}{c}{GAT} & \multicolumn{4}{c}{GCN2} \\
        \midrule
          &   Cora & CiteSeer & CoraFull & CoauthorCS & Cora & CiteSeer & CoraFull & CoauthorCS\\
       \midrule 
       R  &  49.36 (0.52) & 43.53 (0.75) & 9.55 (0.03) & 43.25 (1.1) &  31.53 (0.86) & 37.29 (0.85) & 10.98 (0.08) & 52.61 (0.46) \\
       ID  & 54.08 (0.24) & 44.65 (0.66) & 10.50 (0.04) & 47.30 (0.61) & 31.19 (0.95) & 38.88 (0.86) & 10.40 (0.07) & 54.70 (0.51)\\
       IC & 56.29 (0.28) & 39.19 (0.71) & 11.45 (0.03) & 47.79 (0.72) & 25.79 (0.94) & 39.34 (0.65) & 11.09 (0.11) & 55.86 (0.49) \\
       ICC  & 49.30 (0.32) & 42.40 (0.86) & 10.10 (0.03) & 40.75 (0.43) & 28.30 (0.53) & 32.09 (0.71) & 11.26 (0.06) & 46.66 (0.71) \\
       OURS  &   \textbf{62.76 (0.18)} & \textbf{51.11 (0.07)} & \textbf{13.39 (0.00)}  & \textbf{51.21  (0.11)}  & \textbf{35.61 (0.37)} & \textbf{44.50 (0.04)} & \textbf{15.19 (0.00)}  & \textbf{60.76  (0.02)} \\
    \bottomrule
    \end{tabular}%
    
   }
  \label{tab:init_label}%
\end{table*}%



%\js{Maybe we should remove this minimum cover size optimization formulation? as we didn't conduct any experiment to validate this. It is an application but seems a bit dangling.}

%In addition to finding an initial set of given size $k$, 
% As another application of our locality results, similar principles can be adopted to decide the minimal size of the initial labelled dataset for certain guarantee on the performance of the trained model. A lower bound of the initial labelled set size can be computed by solving the following problem:
% \begin{equation}\label{eq:partial_cover}
% 	\begin{split}
% 		& \min_{\mathcal{D} \subset V} |\mathcal{D}| \\
% 		s.t.&   \sum_{u \in \mathcal{V} \setminus \mathcal{D}} I_r(u|\mathcal{D})  \geq g |\mathcal{V}| \\
% 	\end{split}
% \end{equation}
% where $g \in [0,1]$ and $I_r(u|\mathcal{D})$ is the same indicator function as defined earlier. For a given $r$ and $g$, problem (\ref{eq:partial_cover}) finds the minimum cover which covers at least $g$ portion of all the vertexes within its radius-$r$ neighbourhood. Adjusting the ratio $g$ and radius $r$ controls the performance guarantee resulting from the initial set selection. (\ref{eq:partial_cover}) can be reduced to a minimal partial covering problem
% which is NP-hard, with efficient approximation algorithms available~\citep{partial_cover}. 
% We provide a detailed reduction in Appendix~\ref{appendix:partial_cover}.




% \begin{comment}
% \begin{theorem}\label{thereom:min_cover_ip}
%  Eq.~\eqref{eq:max_cover} can be reduced to the integer programming problem.
% \end{theorem}

% In Appendix~\ref{appdix:}, we provide a detail reduction of Eq.~\eqref{eq:max_cover} to the integer programming problem. This implies that standard techniques/heuristic/analysis used for integer programming can also be applied here. 
% \end{comment}
% \begin{equation}\label{eq:min_cover_ip}
% 	\begin{split}
% 		& \min \sum_{v \in \mathcal{V}} X_v\\
% 		s.t.&  \sum_{v \in N_r(u)} X_v \geq y_v\\
% 		    & \sum_{v \in V} y_v \geq g \|V\| \\
% 		    & y_v \in \{0,1\}\\
% 		    & X_v \in \{0,1\}
% 	\end{split}
% \end{equation}
% where $X_v$ is the indicator variable whether $v$ is selected in the cover.

 




% \begin{equation}
%     \begin{split}
%         P(v) \propto \frac{1}{\text{degree}}
%     \end{split}
% \end{equation}

% \begin{equation}\label{eq:trainSet_selection2}
% 	\begin{split}
% 		& \min \sum_{v \in \mathcal{V}} c_v * X_v\\
% 		s.t.&  \sum_{u \in N_r(v)} X_u \geq 1, \forall v \in \mathcal{V}\\
% 		    & X_v \in \{0,1\}
% 	\end{split}
% \end{equation}
% where $c_v = \frac{1}{\text{deg(v)}}$. 

% \begin{table}[htbp]
% \vspace{-4mm}
%   \centering
%   \caption{Model accuracy of different models trained on Cora. An initial labelled set (k=10) is selected by different strategies, and test set includes the rest of labelled vertexes. We run each strategy 10 times on each model and compute average test accuracy and variance (in brackets). `Cover' is our strategy that solves (\ref{eq:max_cover}) with $r=2$.
%   }  
%     \begin{tabular}{cllll}
%     \toprule
%           &        GCN   & GraphSAGE   & GAT \\
    

         
%     \midrule
%     Random  & 37.08 (0.41) & 37.69 (0.39) & 49.36 (0.52) \\
    
%     \midrule
%     Importance:Degree  & 40.87 (0.38)  & 38.04 (0.40) & 54.08 (0.24)\\
    
%     \midrule
%     Importance:Random Walk  & 39.48 (0.60)  & 38.16 (0.72) & 48.38 (0.19)\\
    
%     \midrule
%     Importance:Centrality  & 37.81 (1.23)  & 42.11 (1.25) & 56.29 (0.28)\\
    
%     \midrule
%     Importance:Cluster Coefficient  & 40.90 (0.39)  & 38.92 (0.29) & 49.30 (0.32)\\
    
          
%     \midrule
%     Cover  & \underline{49.03 (0.05)} & \underline{58.57 (0.01)} & \underline{62.76 (0.18)} \\

%     \bottomrule
%     \end{tabular}%
%   \label{tab:init_label}%
% \end{table}%

==> tex_content/paper/locality.tex <==
\section{Locality in the Prediction Power of GNN}\label{sec:locality}


\subsection{Locality around the Training Set}
We start with showing some structures in the embedding space around the vertices in the training set. We make the following assumptions for our theoretical analysis.
\begin{assumption}[local curvature]\label{assp:local_curvation}
	For all representations $h \in \embdingSpace$, %we assume that
	$\frac{d}{dh}\loss (f(h))$ and $\frac{d^2}{d^2h}\loss (f(h))$ exist, and are continuous and bounded.
\end{assumption}
\begin{assumption}[separability]\label{assp:separability}
    Let $\mathcal{X}_v = \{x_u | u \in \mathcal{N}(v) \cup \{v\}\}$ denote the set of feature vectors from vertex $v$ and its direct neighbors. For a given training set $\mathcal{D}$, we assume that for any $v,u \in \mathcal{D}$ such that $y_u \neq y_v$, we have $\mathcal{X}_v \neq \mathcal{X}_u$. 
\end{assumption}
Assumption~\ref{assp:local_curvation} ensures  
smoothness in the embedding space with respect to the loss function and is a standard technical assumption to make the analysis feasible. Assumption~\ref{assp:separability} guarantees separability among different classes of data and commonly holds in the context where node features are reasonably large and capture a good amount of information. For example, in contexts such as social networks or citation networks, it is very rare for two vertices 
to have the same node features but different labels, and even so for two ego graphs (vertex and its 1-hop neighbors). We further verify this assumption in the experiments in Sec.~\ref{sec:experiment} on commonly used GNN datasets.

Our first result below gives a local structure in the inference performance of GNNs, around vertices in the training set in the embedding space. The detailed proof of all the theorems in this paper can be found in the supplemental material.
\begin{theorem}\label{prop:local_structure}
    Let $\gnnModel$ be a GNN model trained on the vertex set $\mathcal{D}$ with injective property. Let $f$ be a prediction function with sufficient parameters. Under Assumptions~\ref{assp:local_curvation} and~\ref{assp:separability}, there exists $\theta_{\mathcal{D}}$ such that for any $v \in \mathcal{D}$ and $h_v = \gnnModel_{\theta_{\mathcal{D}}}(v)$,  there exists $r_v > 0$ such that for vectors $h,h' \in \embdingSpace$, if
	$d(h,h_v) < d(h',h_v) < r_v$,
	then %we have
	$\loss (h) < \loss (h').$
\end{theorem}

Theorem~\ref{prop:local_structure} states that for each vertex $v$ in the training set, there exists a local neighbourhood of positive radius $r_v$ surrounding representation $h_v$ of $v$ in the embedding space, in which the inference performance (loss) admits simple monotonicity with respect to the distance between the representation of the node and the representation of $v$. This result suggests that if we look at the landscape of the loss function from the perspective of the embedding space, the representation of each vertex in the training set induces a ``valley'' effect in the prediction performance (lowest loss at $h_v$ within the neighbourhood), where losses incurred by representations 
nearby are larger if the respective distance to $h_v$ is larger. 
Fig.~\ref{fig:local_behavior} gives an illustration. 

\begin{remark}
    Theorem~\ref{prop:local_structure} has a surprising connection with the deep learning spline theory~\cite{spline_theory}. It is formally shown in ~\cite{spline_theory} that the learning process of DNN in classification is to cut the input/latent space into a power diagram with small circles, where the representations in each small circle are grouped and classified into the same category. In addition, representations closer to the center of the circle are predicted with more confidence. Theorem~\ref{prop:local_structure} suggests that with GNNs, the centers of the small circles in the power diagram are largely induced by the vertices in the training set.
\end{remark}

\begin{figure*}[t]
 \vspace{-5mm}
\begin{centering}
  \hspace{20mm}  \includegraphics[width=12.5cm,height=5cm,keepaspectratio]{figure/framework/locality.png}
\end{centering}
 \caption{Locality of GNN performance induced by %vertices in training set.
 training vertices. Vertex $a$ is mapped
 to embedding $h_a$. The colored circle in the embedding space represents a neighbourhood centered at $h_a$. Color density represents the loss value: the darker, % the color is,
 the lower the loss is (local minimal loss occurs at $h_a$).
 }
 \vspace{-2mm}
  \label{fig:local_behavior}
\end{figure*}



==> tex_content/paper/preliminary.tex <==
\subsection{Preliminaries}\label{sec:preliminary}

Let $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \featureSet)$ be an undirected graph where $\mathcal{V} = \{1, 2, . . . , N\}$ is the set of $N$ nodes and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ is the set of edges. Let
$\featureSet = \{x_1, x_2, . . . , x_N \}$ denote the set of node attribute vectors corresponding to all the nodes in $\vertexSet$. More specifically, $x_v \in  \featureSet$ is an M-dimensional vector which captures the attribute values of node $v \in \vertexSet$. In addition, each vertex $v \in \mathcal{V}$ is associated with a node label $y_v \in \{1,...,c\}$, where $c$ is the total number of classes.  


For our analysis, we focus on the transductive node classification setting~\cite{transductive} , where the graph $\graph$ are observed prior to learning, and every quantity of interest in the analysis will be conditioned on $\graph$. Without loss of generality, we treat $\graph$ as fixed throughout our analysis and the randomness comes from the labels $y$.  where labels are only available for a small subset of nodes $\vertexSet_0 \subset \mathcal{V}$. We assume that there is at least one labelled vertex in $\mathcal{D}$ for each class. The objective of the semi-supervised node classification task is to learn an embedding function that maps a vertex $v$ (with corresponding inputs) to a representation vector $h_v$, such that $v$'s label can be predicted as $y_v = f(h_v)$, where $f$ is the prediction function. We want the embedding and prediction functions to generalize well to the rest of the vertexes in the graph. 


Given a small set of the labeled nodes, V0 ⊆ V , the task of node-level semi-supervised learning is to learn a classifier h : RN×D × GN → RN×K from a function family H and perform it on the remaining unlabeled nodes. Given a classifier h, the classification for a node i is obtained by



Modern GNNs adopt a neighbourhood aggregation scheme, where the representation of a node is learnt iteratively by aggregating representations of its neighbours. After k iterations of aggregation, a node's representation captures the information within its k-hop neighbourhood in the graph. Formally, the k-th layer of a GNN can be written as follows,
\begin{equation}
    h_{u}^{(k)} = \text{Aggregate}^{(k)}(\{h_v^{(k-1)}, \forall v \in \mathcal{N}(u) \cup \{u\} \}),
\end{equation}
where $h_u^{(k)}$ is the representation vector of node u at the k-th layer. $h_u^{(0)}$ is initialized to be $x_u$, and $\mathcal{N}(u)$ is the set of nodes directly adjacent to $u$. Different GNNs are compositions of aggregation layers of different designs. A GNN is commonly interpreted as an embedding function that combines the graph structure and node features to learn a representation vector $h_v$ of node $v$. Then the learnt representation is fed into a task-specific decoder function $f$ for the prediction. $f$ can be a multilayer perceptron (MLP), a model from another ML family or a deterministic function. 


Let $\embdingSpace \subseteq \oneDimSpace{n}$ be the embedding space of the learnt representations of vertexes and $n \in \mathds{N}$ is the dimension. Let $\gnnModel_{\theta}: \vertexSet \mapsto \embdingSpace$ denotes the GNN model with parameter $\theta$ that maps a vertex $v \in \mathcal{V}$ to a representation vector $h_v$ in the embedding space $\embdingSpace$, following a neighborhood aggregation scheme. Let $f: \embdingSpace \mapsto \oneDimSpace{c}$ be the prediction function that maps an embedding vector $h_v$ to a label $y_v$ in the label set. Then, the GNN prediction process can be viewed as composition of $f \circ \gnnModel_{\theta}: \vertexSet \mapsto \oneDimSpace{c}$. Let $\loss:\oneDimSpace{c} \mapsto \mathds{R}_+$ denote the loss function which evaluates how accurate the prediction is. 











% \section{Preliminaries}\label{sec:preliminary}
% \subsection{Semi-supervised Node Classification}

% Let $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ be an undirected graph where $\mathcal{V} = \{1, 2, . . . , N\}$ is the set of $N$ nodes and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ is the set of edges. Each vertex $v \in \mathcal{V}$ is associated with a $l$-dimensional node feature vector $x_v \in \mathds{R}^{l}$ and can have a node label $y_v \in \{1,...,c\}$, where $c$ is the total number of classes.  For our analysis, we assume $\mathcal{G}$ is connected and we focus on the semi-supervised node classification setting where labels are only available for a small subset of nodes $\mathcal{D} \subset \mathcal{V}$. We assume that there is at least one labelled vertex in $\mathcal{D}$ for each class. The objective of the semi-supervised node classification task is to learn an embedding function that maps a vertex $v$ (with corresponding inputs) to a representation vector $h_v$, such that $v$'s label can be predicted as $y_v = f(h_v)$, where $f$ is the prediction function. We want the embedding and prediction functions to generalize well to the rest of the vertexes in the graph. 






% \subsection{Graph Neural Network}
% \label{sec:gnn_preliminaries}
% Modern GNNs adopt a neighbourhood aggregation scheme, where the representation of a node is learnt iteratively by aggregating representations of its neighbours. After k iterations of aggregation, a node's representation captures the information within its k-hop neighbourhood in the graph. Formally, the k-th layer of a GNN can be written as follows,
% \begin{equation}
%     h_{u}^{(k)} = \text{Aggregate}^{(k)}(\{h_v^{(k-1)}, \forall v \in \mathcal{N}(u) \cup \{u\} \}),
% \end{equation}
% where $h_u^{(k)}$ is the representation vector of node u at the k-th layer. $h_u^{(0)}$ is initialized to be $x_u$, and $\mathcal{N}(u)$ is the set of nodes directly adjacent to $u$. Different GNNs are compositions of aggregation layers of different designs. A GNN is commonly interpreted as an embedding function that combines the graph structure and node features to learn a representation vector $h_v$ of node $v$. Then the learnt representation is fed into a task-specific decoder function $f$ for the prediction. $f$ can be a multilayer perceptron (MLP), a model from another ML family or a deterministic function. 


% Let $\embdingSpace \subseteq \oneDimSpace{n}$ be the embedding space of the learnt representations of vertexes and $n \in \mathds{N}$ is the dimension. Let $\gnnModel_{\theta}: \vertexSet \mapsto \embdingSpace$ denotes the GNN model with parameter $\theta$ that maps a vertex $v \in \mathcal{V}$ to a representation vector $h_v$ in the embedding space $\embdingSpace$, following a neighborhood aggregation scheme. Let $f: \embdingSpace \mapsto \oneDimSpace{c}$ be the prediction function that maps an embedding vector $h_v$ to a label $y_v$ in the label set. Then, the GNN prediction process can be viewed as composition of $f \circ \gnnModel_{\theta}: \vertexSet \mapsto \oneDimSpace{c}$. Let $\loss:\oneDimSpace{c} \mapsto \mathds{R}_+$ denote the loss function which evaluates how accurate the prediction is. 










==> tex_content/paper/regularization.tex <==
\section{Fair-GNN Framework}
In the previous sections, we have formally shown that GNNs have unfair prediction power with respect to the spatial-distance of vertices to the training set. We have also shown that the reason for this unfair prediction power is the low distortion rate between graph domain and the embedding domain, i.e., vertices closers in the graph domain are also closer in the embedding domain. Based on this insight, we propose a fairness regularizer that aims to break the continum  between graph distance and the embedding distance. 

To do that, we randomly sample a set vertices outside of the training set and test set and refer to this set as the anchor set. The idea of this anchor set is to provide a random spatial reference to the training set in the graph domain. Then, we can regularize the prediction power of GNNs by controlling the distance between the representations of the training set to the representations of this sampled anchor set.

More formally, let $\mathcal{I}$ be the randomly selected anchor set. Let $\mathcal{Z}_{tr}$ be the represnetation of the training set and let $\mathcal{Z}_{\mathcal{I}}$ be the set of representation of the anchor set. Then, the training objective of our fairness regularization is 

\begin{equation}
    \mathcal{L}_{fair} = \beta \mathcal{L}_{c}(D_{tr}) + \alpha d(Z_{tr},Z_{\mathcal{I}}).
\end{equation}
